Density profiles in a classical Coulomb fluid near a dielectric wall. II. Weak-coupling systematic expansions

In the framework of the grand-canonical ensemble of statistical mechanics, we give an exact diagrammatic representation of the density profiles in a classical multicomponent plasma near a dielectric wall. By a reorganization of Mayer diagrams for the fugacity expansions of the densities, we exhibit how the long-range of both the self-energy and pair interaction are exponentially screened at large distances from the wall. However, the self-energy due to Coulomb interaction with images still diverges in the vicinity of the dielectric wall and the variation of the density is drastically different at short or large distances from the wall. This variation is involved in the inhomogeneous Debye-H\"uckel equation obeyed by the screened pair potential. Then the main difficulty lies in the determination of the latter potential at every distance. We solve this problem by devising a systematic expansion with respect to the ratio of the fundamental length scales involved in the two coulombic effects at stake. (The application of this method to a plasma confined between two ideally conducting plates and to a quantum plasma will be presented elsewhere). As a result we derive the exact analytical perturbative expressions for the density profiles up to first order in the coupling between charges. The mean-field approach displayed in Paper I is then justified.

==> Figure/Fig1 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 2 0 0 100 0 -1 0.000 1 0.0000 2025 2925 212 212 2025 2925 2237 2925
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 1200 2100 106 106 1200 2100 1306 2100
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 3450 2925 106 106 3450 2925 3556 2925
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 5025 2925 106 106 5025 2925 5131 2925
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 4275 3600 106 106 4275 3600 4381 3600
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 4200 2250 106 106 4200 2250 4306 2250
1 3 0 2 0 0 100 0 -1 0.000 1 0.0000 8100 2925 212 212 8100 2925 8312 2925
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 7200 2025 106 106 7200 2025 7306 2025
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 9525 2925 106 106 9525 2925 9631 2925
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 10425 3600 106 106 10425 3600 10531 3600
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 10350 2250 106 106 10350 2250 10456 2250
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 11144 2925 106 106 11144 2925 11250 2925
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 3675 1800 106 106 3675 1800 3781 1800
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 4200 1306 106 106 4200 1306 4306 1306
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 4725 1725 106 106 4725 1725 4831 1725
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 11700 2400 106 106 11700 2400 11806 2400
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 12194 2850 106 106 12194 2850 12300 2850
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 11700 3375 106 106 11700 3375 11806 3375
1 3 0 2 0 0 100 0 -1 0.000 1 0.0000 17250 2850 212 212 17250 2850 17462 2850
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 16350 1950 106 106 16350 1950 16456 1950
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 18675 2850 106 106 18675 2850 18781 2850
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 19500 2131 106 106 19500 2131 19606 2131
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 19575 3525 106 106 19575 3525 19681 3525
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 20369 2850 106 106 20369 2850 20475 2850
2 1 1 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 1200 2100 1875 2775
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 2250 2850 3375 2850
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 2250 3000 3375 3000
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 3450 2925 4200 2250
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 4200 2250 5025 2925
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 4256 3579 5006 2904
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 3453 2921 4278 3596
2 1 1 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 7275 2100 7950 2775
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 8325 3000 9450 3000
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 8325 2850 9450 2850
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 9585 2908 10335 2233
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 9580 2949 10405 3624
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 10410 3583 11160 2908
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 10302 2217 11127 2892
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 6
	 4125 2175 3675 1800 4200 1275 4725 1725 4275 2175 4200 2250
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 6
	 11625 3300 11175 2925 11700 2400 12225 2850 11775 3300 11700 3375
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 1 0 2
	2 1 3.00 120.00 150.00
	 13125 2850 15525 2850
2 1 1 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 16425 2025 17100 2700
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 17475 2775 18600 2775
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 17475 2925 18600 2925
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 18735 2758 19485 2083
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 18723 2882 19548 3557
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 19560 3508 20310 2833
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 19527 2142 20352 2817
4 0 0 100 0 3 154 0.0000 0 240 345 6150 3000 +\001
4 0 0 100 0 3 100 0.0000 0 345 240 3225 3450 1\001
4 0 0 100 0 3 100 0.0000 0 345 240 4125 4125 2\001
4 0 0 100 0 3 100 0.0000 0 345 240 5175 3300 3\001
4 0 0 100 0 3 100 0.0000 0 345 240 3600 2475 4\001
4 0 0 100 0 3 100 0.0000 0 345 240 975 1725 5\001
4 0 0 100 0 3 100 0.0000 0 345 240 7275 1800 5\001
4 0 0 100 0 3 100 0.0000 0 345 240 9300 3450 1\001
4 0 0 100 0 3 100 0.0000 0 345 240 10275 4200 2\001
4 0 0 100 0 3 100 0.0000 0 345 240 9900 2025 4\001
4 0 0 100 0 3 100 0.0000 0 345 240 11025 3525 3\001
4 0 0 100 0 3 100 0.0000 0 345 240 16425 1650 5\001
4 0 0 100 0 3 100 0.0000 0 345 240 19050 1800 4\001
4 0 0 100 0 3 100 0.0000 0 345 240 20700 3075 3\001
4 0 0 100 0 3 100 0.0000 0 345 240 19575 4125 2\001
4 0 0 100 0 3 100 0.0000 0 345 240 18525 3450 1\001
4 0 0 100 0 3 102 0.0000 0 345 360 8550 5625 G\001
4 0 0 100 0 3 102 0.0000 0 345 360 2550 5625 G\001
4 0 0 100 0 3 80 0.0000 0 345 300 2850 5775 A\001
4 0 0 100 0 3 80 0.0000 0 345 300 9000 5850 A\001
4 0 0 100 0 3 80 0.0000 0 225 240 3300 6000 a\001
4 0 0 100 0 3 80 0.0000 0 225 240 9450 6075 a\001
4 0 0 100 0 3 102 0.0000 0 345 360 17850 5625 G\001
4 0 0 100 0 3 80 0.0000 0 345 300 18225 6075 A\001
4 0 0 100 0 3 60 0.0000 0 195 255 18225 5400 *\001
4 0 0 100 0 3 60 0.0000 0 195 255 8925 5400 *\001
4 0 0 100 0 3 60 0.0000 0 195 255 2925 5400 *\001
4 0 0 100 0 3 40 0.0000 0 435 630 18600 5175 [0]\001


==> Figure/Fig2 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 10050 2850 106 106 10050 2850 10156 2850
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 10950 3525 106 106 10950 3525 11056 3525
1 3 0 2 0 0 100 0 -1 0.000 1 0.0000 8625 2850 212 212 8625 2850 8837 2850
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 7694 1950 106 106 7694 1950 7800 1950
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 10950 2025 106 106 10950 2025 11056 2025
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 11850 2775 106 106 11850 2775 11956 2775
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 6031 2775 106 106 6031 2775 6137 2775
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 5175 2025 106 106 5175 2025 5281 2025
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 5175 3525 106 106 5175 3525 5281 3525
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 4275 2850 106 106 4275 2850 4381 2850
1 3 0 2 0 0 100 0 -1 0.000 1 0.0000 2850 2850 212 212 2850 2850 3062 2850
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 1985 1950 106 106 1985 1950 2091 1950
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 8850 2925 9975 2925
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 8850 2775 9975 2775
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 10110 2758 10860 2083
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 10108 2882 10933 3557
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 11003 3508 11753 2833
2 1 1 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 7800 2025 8475 2700
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 11032 2072 11857 2747
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 5175 2080 6000 2755
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 5228 3508 5978 2833
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 4359 2882 5184 3557
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 4328 2750 5078 2075
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 3075 2925 4200 2925
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 3075 2775 4200 2775
2 1 1 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 2025 2025 2700 2700
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 5100 3825 5300 3825
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 5100 1425 5300 1425
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 3900 2250 4100 2250
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 2475 3450 2675 3450
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 1950 1350 2150 1350
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 6075 3000 6275 3000
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 6825 2775 7350 2775
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 10800 3900 11000 3900
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 12075 2700 12275 2700
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 10875 1500 11075 1500
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 7650 1425 7850 1425
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 8400 3300 8600 3300
2 1 0 3 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 9600 3300 9800 3300
4 0 0 100 0 3 102 0.0000 0 345 360 75 3000 G\001
4 0 0 100 0 3 80 0.0000 0 345 300 375 3375 A\001
4 0 0 100 0 3 60 0.0000 0 195 255 450 2850 *\001
4 0 0 100 0 3 40 0.0000 0 435 630 675 2550 [1]\001
4 0 0 100 0 3 100 0.0000 0 135 345 1200 3000 =\001
4 0 0 100 0 3 80 0.0000 0 225 195 5100 4200 z\001
4 0 0 100 0 3 80 0.0000 0 225 195 5100 1725 z\001
4 0 0 100 0 3 80 0.0000 0 225 195 3900 2550 z\001
4 0 0 100 0 3 21 0.0000 0 315 480 5400 3900 [1]\001
4 0 0 100 0 3 21 0.0000 0 315 480 4125 2325 [1]\001
4 0 0 100 0 3 21 0.0000 0 315 480 5400 1425 [1]\001
4 0 0 100 0 3 80 0.0000 0 225 195 2475 3750 z\001
4 0 0 100 0 3 21 0.0000 0 315 480 2700 3525 [1]\001
4 0 0 100 0 3 80 0.0000 0 225 195 1950 1650 z\001
4 0 0 100 0 3 21 0.0000 0 315 480 2175 1350 [1]\001
4 0 0 100 0 3 80 0.0000 0 225 195 6075 3300 z\001
4 0 0 100 0 3 21 0.0000 0 315 480 6300 3075 [1]\001
4 0 0 100 0 3 80 0.0000 0 225 195 10800 4200 z\001
4 0 0 100 0 3 80 0.0000 0 225 195 12075 3000 z\001
4 0 0 100 0 3 80 0.0000 0 225 195 10875 1800 z\001
4 0 0 100 0 3 80 0.0000 0 225 195 7650 1725 z\001
4 0 0 100 0 3 21 0.0000 0 315 480 7875 1500 [1]\001
4 0 0 100 0 3 80 0.0000 0 225 195 8400 3600 z\001
4 0 0 100 0 3 21 0.0000 0 315 480 8700 3375 [1]\001
4 0 0 100 0 3 80 0.0000 0 225 195 9600 3600 z\001
4 0 0 100 0 3 21 0.0000 0 315 480 9825 3375 [1]\001


==> Figure/Fig3 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 10050 2850 106 106 10050 2850 10156 2850
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 10950 3525 106 106 10950 3525 11056 3525
1 3 0 2 0 0 100 0 -1 0.000 1 0.0000 8625 2850 212 212 8625 2850 8837 2850
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 10950 2025 106 106 10950 2025 11056 2025
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 11850 2775 106 106 11850 2775 11956 2775
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 6031 2775 106 106 6031 2775 6137 2775
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 5175 2025 106 106 5175 2025 5281 2025
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 5175 3525 106 106 5175 3525 5281 3525
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 4275 2850 106 106 4275 2850 4381 2850
1 3 0 2 0 0 100 0 -1 0.000 1 0.0000 2850 2850 212 212 2850 2850 3062 2850
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 1985 1950 106 106 1985 1950 2091 1950
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 3119 3375 106 106 3119 3375 3225 3375
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 3975 3375 106 106 3975 3375 4081 3375
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 5550 2400 106 106 5550 2400 5656 2400
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 3000 1800 106 106 3000 1800 3106 1800
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 8775 1800 106 106 8775 1800 8881 1800
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 7725 2025 106 106 7725 2025 7831 2025
1 3 0 1 0 0 100 0 20 0.000 1 0.0000 10500 2431 106 106 10500 2431 10606 2431
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 8850 2925 9975 2925
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 8850 2775 9975 2775
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 10110 2758 10860 2083
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 10108 2882 10933 3557
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 11003 3508 11753 2833
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 11032 2072 11857 2747
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 5175 2080 6000 2755
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 5228 3508 5978 2833
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 4359 2882 5184 3557
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 4328 2750 5078 2075
2 1 1 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 2025 2025 2700 2700
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 3075 2850 4200 2850
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 4
	 2925 3075 3150 3375 3975 3375 4275 2925
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 3
	 2025 1950 3000 1800 2850 2625
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 3
	 7797 1933 8772 1783 8622 2608
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 7822 2000 8572 2675
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 7672 2075 8422 2750
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 900 300 1200 300
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 3
	 900 300 900 4800 1200 4800
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 3
	 7275 300 7275 4800 7575 4800
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 7275 300 7575 300
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 5
	 6300 375 6525 375 6600 375 6600 4800 6225 4800
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 5
	 12450 300 12675 300 12750 300 12750 4725 12375 4725
4 0 0 100 0 3 102 0.0000 0 345 360 3525 5700 G\001
4 0 0 100 0 3 80 0.0000 0 345 300 3825 6075 A\001
4 0 0 100 0 3 60 0.0000 0 195 255 3975 5550 *\001
4 0 0 100 0 3 40 0.0000 0 435 630 4275 5475 [1]\001
4 0 0 100 0 3 102 0.0000 0 345 360 9450 5700 G\001
4 0 0 100 0 3 60 0.0000 0 195 255 9900 5550 *\001
4 0 0 100 0 3 40 0.0000 0 435 630 10275 5475 [1]\001
4 0 0 100 0 3 80 0.0000 0 345 300 9825 6075 B\001
4 0 0 100 0 3 80 0.0000 0 345 240 3900 3900 8\001
4 0 0 100 0 3 80 0.0000 0 345 240 4200 2550 1\001
4 0 0 100 0 3 80 0.0000 0 345 240 5100 3975 2\001
4 0 0 100 0 3 80 0.0000 0 345 240 6300 2925 3\001
4 0 0 100 0 3 80 0.0000 0 345 240 5100 1650 4\001
4 0 0 100 0 3 80 0.0000 0 345 240 5775 2250 9\001
4 0 0 100 0 3 80 0.0000 0 345 240 3225 1650 6\001
4 0 0 100 0 3 80 0.0000 0 345 240 1800 1575 5\001
4 0 0 100 0 3 80 0.0000 0 345 240 2850 3900 7\001
4 0 0 100 0 3 80 0.0000 0 345 240 7425 1650 5\001
4 0 0 100 0 3 80 0.0000 0 345 240 11175 1800 4\001
4 0 0 100 0 3 80 0.0000 0 345 240 12150 2775 3\001
4 0 0 100 0 3 80 0.0000 0 345 240 10950 3975 2\001
4 0 0 100 0 3 80 0.0000 0 345 240 9000 1575 6\001
4 0 0 100 0 3 80 0.0000 0 345 480 10200 2175 10\001
4 0 0 100 0 3 80 0.0000 0 345 240 9825 3375 1\001
4 0 0 100 0 3 100 0.0000 0 345 270 6600 5175 T\001
4 0 0 100 0 3 100 0.0000 0 345 270 12750 5100 T\001


==> Figure/Fig4 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 2 0 0 100 0 -1 6.000 1 0.0000 3543 3150 168 168 3543 3150 3393 3075
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 5585 3127 106 106 5585 3127 5691 3127
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 2260 1359 106 106 2260 1359 2366 1359
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 4
	 675 2970 600 2970 600 3290 675 3290
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 3375 3075 3150 2850
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 3150 2850 3450 2550
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 3450 2550 3225 2325
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 2925 2625 3225 2325
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 2925 2625 2700 2400
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 2700 2400 3000 2100
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 3000 2100 2775 1875
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 2475 2175 2775 1875
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 2475 2175 2250 1950
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 2250 1950 2550 1650
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 2550 1650 2325 1425
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 3075 3750 3300 3750
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 2025 825 2250 825
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 5850 2850 6075 2850
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 6600 3000 6825 3000
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 6900 2850 7125 2850
3 0 0 2 0 0 100 0 -1 6.000 0 0 0 3
	 3700 3075 4525 2475 5500 3075
	 0.000 1.000 0.000
3 0 0 2 0 0 100 0 -1 6.000 0 0 0 3
	 5462 3090 4637 3690 3662 3090
	 0.000 1.000 0.000
4 0 0 100 0 0 100 0.0000 0 345 270 600 3300 P\001
4 0 0 100 0 1 100 0.0000 0 135 285 1200 3300 =\001
4 0 0 100 0 1 80 0.0000 0 225 225 3075 4050 z\001
4 0 0 100 0 1 21 0.0000 0 315 420 3375 3825 [2]\001
4 0 0 100 0 1 80 0.0000 0 225 225 2025 1125 z\001
4 0 0 100 0 1 21 0.0000 0 315 420 2325 825 [2]\001
4 0 0 100 0 1 80 0.0000 0 225 225 5850 3150 z\001
4 0 0 100 0 1 21 0.0000 0 315 420 6075 2925 [2]\001
4 0 0 100 0 1 80 0.0000 0 225 225 6900 3150 z\001
4 0 0 100 0 1 21 0.0000 0 315 420 7200 2925 [1]\001


==> Figure/Fig5 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 4800 2775 106 106 4800 2775 4906 2775
1 4 0 2 0 0 100 0 -1 0.000 1 0.0000 1645 2754 171 171 1474 2754 1816 2754
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 3225 2775 106 106 3225 2775 3331 2775
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 2400 2775 106 106 2400 2775 2506 2775
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 4019 2775 106 106 4019 2775 4125 2775
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 3675 2175 106 106 3675 2175 3781 2175
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 2775 2175 106 106 2775 2175 2881 2175
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 3225 1575 106 106 3225 1575 3331 1575
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 3225 600 106 106 3225 600 3331 600
1 4 0 2 0 0 100 0 -1 0.000 1 0.0000 7345 2754 171 171 7174 2754 7516 2754
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 10500 2775 106 106 10500 2775 10606 2775
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 8925 2775 106 106 8925 2775 9031 2775
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 8100 2775 106 106 8100 2775 8206 2775
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 9750 2775 106 106 9750 2775 9856 2775
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 8506 2175 106 106 8506 2175 8612 2175
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 9375 2175 106 106 9375 2175 9481 2175
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 8925 1575 106 106 8925 1575 9031 1575
1 4 0 2 0 0 100 0 -1 0.000 1 0.0000 12171 2775 171 171 12000 2775 12342 2775
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 15375 2775 106 106 15375 2775 15481 2775
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 13725 2775 106 106 13725 2775 13831 2775
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 12931 2775 106 106 12931 2775 13037 2775
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 13275 2175 106 106 13275 2175 13381 2175
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 14144 2175 106 106 14144 2175 14250 2175
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 13694 1575 106 106 13694 1575 13800 1575
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 14625 2775 106 106 14625 2775 14731 2775
1 4 0 2 0 0 100 0 -1 0.000 1 0.0000 7345 7350 171 171 7174 7350 7516 7350
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 8925 7350 106 106 8925 7350 9031 7350
1 3 0 2 0 0 100 0 20 0.000 1 0.0000 10500 7350 106 106 10500 7350 10606 7350
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 1800 2760 4800 2760
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 5
	 3225 2775 2775 2175 3225 1575 3675 2175 3225 2775
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 3150 675 3150 1500
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 3300 675 3300 1500
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 1 0 2
	2 1 3.00 60.00 120.00
	 5325 2775 6675 2775
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 7500 2760 10500 2760
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 5
	 8925 2775 8475 2175 8925 1575 9375 2175 8925 2775
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 8925 1050 9150 1050
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 9600 1800 9825 1800
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 7875 1800 8100 1800
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 11025 2775 11400 2775
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 2
	 12365 2775 15375 2775
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 5
	 13713 2775 13263 2175 13713 1575 14163 2175 13713 2775
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 12750 1800 12975 1800
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 14400 1800 14625 1800
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 13725 1050 13950 1050
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 1 0 2
	2 1 3.00 60.00 120.00
	 5325 7350 6675 7350
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 8400 6300 8625 6300
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 9300 6300 9525 6300
2 1 0 2 0 0 100 0 -1 6.000 0 0 -1 0 0 2
	 8850 6450 9150 6450
2 1 0 2 0 0 100 0 -1 0.000 0 0 -1 0 0 4
	 8925 8140 8800 8140 8800 8475 8925 8475
3 2 0 2 0 0 100 0 -1 6.000 0 0 0 6
	 7500 7275 7725 6975 8025 7575 8325 6975 8625 7575 8925 7350
	 0.000 -1.000 -1.000 -1.000 -1.000 0.000
3 2 0 2 0 0 100 0 -1 6.000 0 0 0 6
	 9030 7290 9255 6990 9555 7590 9855 6990 10155 7590 10455 7365
	 0.000 -1.000 -1.000 -1.000 -1.000 0.000
4 0 0 100 0 1 100 0.0000 0 345 360 3075 4650 G\001
4 0 0 100 0 1 40 0.0000 0 195 255 3450 4500 *\001
4 0 0 100 0 1 80 0.0000 0 345 240 2325 3300 1\001
4 0 0 100 0 1 80 0.0000 0 345 240 3150 3300 2\001
4 0 0 100 0 1 80 0.0000 0 345 240 3900 3300 3\001
4 0 0 100 0 1 80 0.0000 0 345 240 4725 3300 4\001
4 0 0 100 0 1 80 0.0000 0 345 240 7950 3300 1\001
4 0 0 100 0 1 80 0.0000 0 345 240 8925 3300 2\001
4 0 0 100 0 1 80 0.0000 0 345 240 9675 3300 3\001
4 0 0 100 0 1 80 0.0000 0 345 240 10350 3300 4\001
4 0 0 100 0 1 60 0.0000 0 225 225 7875 2100 z\001
4 0 0 100 0 1 21 0.0000 0 315 420 8100 1875 [1]\001
4 0 0 100 0 1 60 0.0000 0 225 225 8925 1350 z\001
4 0 0 100 0 1 21 0.0000 0 315 420 9150 1125 [1]\001
4 0 0 100 0 1 60 0.0000 0 225 225 9600 2100 z\001
4 0 0 100 0 1 21 0.0000 0 315 420 9825 1875 [1]\001
4 0 0 100 0 1 80 0.0000 0 345 240 12825 3300 1\001
4 0 0 100 0 1 80 0.0000 0 345 240 13650 3300 2\001
4 0 0 100 0 1 80 0.0000 0 345 240 15300 3300 4\001
4 0 0 100 0 1 80 0.0000 0 345 240 14550 3300 3\001
4 0 0 100 0 1 60 0.0000 0 225 225 12750 2100 z\001
4 0 0 100 0 1 60 0.0000 0 225 225 14400 2100 z\001
4 0 0 100 0 1 60 0.0000 0 225 225 13725 1350 z\001
4 0 0 100 0 1 100 0.0000 0 345 360 11250 4650 G\001
4 0 0 100 0 1 40 0.0000 0 195 255 11625 4500 *\001
4 0 0 100 0 1 21 0.0000 0 315 420 11925 4275 [1]\001
4 0 0 100 0 1 60 0.0000 0 225 225 8400 6600 z\001
4 0 0 100 0 1 21 0.0000 0 315 420 8700 6300 [1]\001
4 0 0 100 0 1 60 0.0000 0 225 225 9300 6600 z\001
4 0 0 100 0 1 21 0.0000 0 315 420 9600 6300 [2]\001
4 0 0 100 0 1 100 0.0000 0 345 270 8850 8475 P\001

